Correlated Link Shadow Fading in Multi-hop Wireless Networks

Accurate representation of the physical layer is required for analysis and simulation of multi-hop networking in sensor, ad hoc, and mesh networks. This paper investigates, models, and analyzes the correlations that exist in shadow fading between links in multi-hop networks. Radio links that are geographically proximate often experience similar environmental shadowing effects and thus have correlated fading. We describe a measurement procedure and campaign to measure a large number of multi-hop networks in an ensemble of environments. The measurements show statistically significant correlations among shadowing experienced on different links in the network, with correlation coefficients up to 0.33. We propose a statistical model for the shadowing correlation between link pairs which shows strong agreement with the measurements, and we compare the new model with an existing shadowing correlation model of Gudmundson (1991). Finally, we analyze multi-hop paths in three and four node networks using both correlated and independent shadowing models and show that independent shadowing models can underestimate the probability of route failure by a factor of two or greater.

==> abstract_new.tex <==
Radio links that are geographically proximate often experience similar environmental shadowing effects. This paper investigates, models, and analyzes the correlations that exist in shadowing between links in multi-hop networks. We conduct extensive measurements which show statistically significant correlations among shadowing on different links in a multi-hop network, with correlation coefficients up to 0.33. We present a measurement-verified model for correlated shadowing, and compare with an existing model of Gudmundson (1991). Finally, we analyze simple multi-hop networks and show that independent shadowing models underestimate route failure probabilities by a factor of two or greater. 
